Inference on quantile processes with a finite number of clusters

I introduce a generic method for inference on entire quantile and regression quantile processes in the presence of a finite number of large and arbitrarily heterogeneous clusters. The method asymptotically controls size by generating statistics that exhibit enough distributional symmetry such that randomization tests can be applied. The randomization test does not require ex-ante matching of clusters, is free of user-chosen parameters, and performs well at conventional significance levels with as few as five clusters. The method tests standard (non-sharp) hypotheses and can even be asymptotically similar in empirically relevant situations. The main focus of the paper is inference on quantile treatment effects but the method applies more broadly. Numerical and empirical examples are provided.

==> macros.tex <==
\numberwithin{equation}{section}
%\allowdisplaybreaks

%\swapnumbers

%\renewcommand\thesubsection {\bfseries\thesection.\arabic{subsection}}
%\renewcommand{\hat}{\widehat}

\makeatletter
\def\swappedhead#1#2#3{%
  % original definition:
  % \thmnumber{\@upn{\the\thm@headfont#2\@ifnotempty{#1}{.~}}}%
  % change:
  \thmnumber{\@upn{\the\thm@headfont#2\@ifnotempty{#1}{.~}}}%
  \thmname{#1}%
  \thmnote{ {\the\thm@notefont(#3)}}}
\makeatother

\makeatletter
\def\th@plain{%
  \thm@notefont{}% same as heading font
  \itshape % body font
}
\def\th@definition{%
  \thm@notefont{}% same as heading font
  \normalfont % body font
}
\makeatother

\makeatletter
\renewcommand*\@adminfootnotes{%
  \let\@makefnmark\relax  \let\@thefnmark\relax
  \ifx\@empty\@date\else \@footnotetext{\@setdate\ \def\par{\let\par\@par}\@setthanks}\fi%
  \ifx\@empty\@subjclass\else \@footnotetext{\@setsubjclass}\fi
  \ifx\@empty\@keywords\else \@footnotetext{\@setkeywords}\fi
  %\ifx\@empty\thankses\else \@footnotetext{%
  %  \def\par{\let\par\@par}\@setthanks}%
  %\fi
}
\makeatother

\oddsidemargin +0.2in \evensidemargin +0.2in \topmargin 40pt \textheight 8.1in \textwidth 6in %\linespread{1.3} 
%\parskip .03in
\usepackage{setspace}
\setstretch{1.5}
%\usepackage[paperwidth = 6.5in, textwidth = 5.05in]{geometry}

\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}

\usepackage[font=footnotesize]{caption}
